All That Glitters Is Not Gold: Towards Process Discovery Techniques with Guarantees

The aim of a process discovery algorithm is to construct from event data a process model that describes the underlying, real-world process well. Intuitively, the better the quality of the event data, the better the quality of the model that is discovered. However, existing process discovery algorithms do not guarantee this relationship. We demonstrate this by using a range of quality measures for both event data and discovered process models. This paper is a call to the community of IS engineers to complement their process discovery algorithms with properties that relate qualities of their inputs to those of their outputs. To this end, we distinguish four incremental stages for the development of such algorithms, along with concrete guidelines for the formulation of relevant properties and experimental validation. We will also use these stages to reflect on the state of the art, which shows the need to move forward in our thinking about algorithmic process discovery.

==> section/casestudy.tex <==
To illustrate the different stages of designing a process discovery algorithm, we apply it on the Inductive Miner~\cite{LeemansFA14}.
For the first stage, the designers of the algorithm have to set the class of true processes it focuses on: \emph{process trees}. 
The goal of the algorithm is \emph{rediscoverability}: if for some process tree, a ``activity-complete'' event log is provided, then the original process tree is discovered by the algorithm.
The authors prove their algorithm correct under the assumption that a log is directy-follows-complete, i.e., if all directly-follows relations of the true process are be present in the event log, then the normal form of the original model can be discovered.
Hence, \cite{LeemansFA14} fulfills all criteria for stage 1. 

For stage 2, the algorithm should be validated on a set of real-life event logs. 
In~\cite{LeemansFA15}, the authors show the scalability of their approach.
Experiments are performed on several large test data sets, and on the BPI Challenge log 2012~\cite{Dongen2012}.

Case Study on a State-of-the-Art Process Discovery Algorithm

AS AN EXAMPLE, WE TAKE THE INDUCTIVEMINER

STAGE 1. DESIGN THE ALGORITHM

A. IT DESCRIBES THE CLASS OF PROCESS MODELS THE ALGORITHM AIMS TO DISCOVER:

PROCESS TREES

b. IT DEFINES THE CORRECTNESS GOAL OF THE ALGORITHM

REDISCOVERABILITY

STAGE 2. VALIDATE THE ALGORITHM ON REAL-LIFE EXAMPLE

\subsection{In Vivo: Sampling To Validate Process Discovery Results}
Two real-life event logs have been chosen for the in-vivo experiment, the Road Traffic Fine management process event log~\cite{deLeoni2015}, and the Sepsis cases event log~\cite{Mannhardt2016}.
These event logs have been chosen based on their dissimilar properties.
The Road Fine log has in total 150,370 traces and 561,470 events.
There are 231 unique traces and 11 unique event types.
The Sepsis log consists of 1,049 traces, of which 845 are unique, and 15,190 events with 16 unique event types.

Sampling was done at twelve different sampling ratios: $0.01$, $0.02$, $0.05$, and $0.1$ up to $0.9$.
For each ratio, 10 samples were drawn.
To validate the hypothesis that better samples result in higher precision models, Spearman's correlation is calculated for each error measure.
In this experiment, we applied simple random sampling to generate samples.

The sample quality measures for the Road Fine Log are shown in Fig.~\ref{fig:road-ratio-error}.
As the plot shows, the larger the sampling ratio, and thus the log size, the smaller the error is (for all measures: $\rho < -0.9$, $p < 0.001$).
Sample size and the conformance measure on precision (Fig.~\ref{fig:road-ratio-precision}) shows a moderate positive correlation ($\rho=0.56$, $p < 0.001$), while there is no correlation between sampling ratio and recall ($\rho=0.03$, $p=0.72$).
Analyzing the error measures with the conformance measures shows a different story.
In Fig.~\ref{fig:road-error-precision}, the error measure sMAPE is plot against the precision.
As the plot already indicates, no correlations are found between the error measures and precision (sMAPE: $\rho = -0.19$, $p=0.03$, sRMSPE: $\rho = -0.18$, $p=0.051$, NRMSE: $\rho = -0.21$, $p=0.02$, and NMAE: $\rho = -0.20$, $p=0.03$).
Recall even shows a positive correlation with the error measures (sMAPE: $\rho = 0.80$, $p<0.001$, sRMSPE: $\rho = 0.79$, $p< 0.001$, NRMSE: $\rho = 0.77$, $p<0.001$, and NMAE: $\rho = 0.78$, $p < 0.001$).
Coverage has no correlation with precision ($\rho = 0.17$, $p=0.06$) and a negative correlation with recall ($\rho=-0.79$, $p<0.001$).

\begin{figure}
	\begin{minipage}{.47\textwidth}
		\resizebox{\columnwidth}{!}{\input{images/road_errors_ratio.tex}}
		\caption{Plot of ratio and the sample quality measures coverage ($\bullet$), sMAPE ($+$), sRMSPE ($\boxtimes$), NRMSE ($\blacksquare$) and NMAE ($\blacktriangle$) for the Road Fine Log }\label{fig:road-ratio-error}
	\end{minipage}
	\hfill
	\begin{minipage}{.47\textwidth}
		\resizebox{\columnwidth}{!}{\input{images/sepsis_errors_ratio.tex}}
		\caption{Plot of ratio and the sample quality measures coverage ($\bullet$), sMAPE ($+$), sRMSPE ($\boxtimes$), NRMSE ($\blacksquare$) and NMAE ($\blacktriangle$) for the Sepsis Log}\label{fig:sepsis-ratio-error}
	\end{minipage}
	\begin{minipage}{.47\textwidth}
		\resizebox{\columnwidth}{!}{\input{images/road_precision_ratio.tex}}
		\caption{Plot of ratio and precision of the Road log}\label{fig:road-ratio-precision}
	\end{minipage}
	\hfill
	\begin{minipage}{.47\textwidth}
		\resizebox{\columnwidth}{!}{\input{images/sepsis_precision_ratio.tex}}
		\caption{Plot of ratio and precision of the Sepsis log}\label{fig:sepsis-ratio-precision}
	\end{minipage}
	\begin{minipage}{.47\textwidth}
		\resizebox{\columnwidth}{!}{\input{images/road_precision_coverage.tex}}
		\resizebox{\columnwidth}{!}{\input{images/road_recall_coverage.tex}}
		\caption{Plot of sMAPE and precision recall of the Road log}\label{fig:road-error-precision}
	\end{minipage}
	\hfill
	\begin{minipage}{.47\textwidth}
		\resizebox{\columnwidth}{!}{\input{images/sepsis_precision_coverage.tex}}
		\resizebox{\columnwidth}{!}{\input{images/sepsis_recall_coverage.tex}}
		\caption{Plot of NRMSE and precision of the Sepsis log}\label{fig:sepsis-error-precision}
	\end{minipage}
\end{figure}

%RESULT SEPSIS LOG
For the Sepsis Log, similar results are found.
As indicated by Fig.~\ref{fig:sepsis-ratio-error}, a strong correlation is found between the sampling ratio and the error measures (for all measures: $\rho < -0.9$, $p < 0.001$).
The larger the sampling ratio, the higher the precision is ($\rho=0.57$, $p< 0.001$), but
no correlation was found between sampling ratio and recall ($\rho=0.03$, $p=0.72$).
A moderate negative correlation was found between the error measures and precision
(sMAPE: $\rho = -0.58$, $p<0.001$, sRMSPE: $\rho = -0.59$, $p< 0.001$, NRMSE: $\rho = -0.52$, $p<0.001$, and NMAE: $\rho = -0.54$, $p < 0.001$), while the error measures with recall did not show any correlation
(sMAPE: $\rho = -0.02$, $p=0.82$, sRMSPE: $\rho = -0.01$, $p=0.92$, NRMSE: $\rho = -0.03$, $p=0.72$, and NMAE: $\rho = -0.03$, $p=0.75$).
Coverage had a moderate correlation with precision ($\rho = 0.59$, $p < 0.001$) and no correlation with recall ($\rho=0.01$, $p=0.96$).

\subsection{In Vitro: Validating Discovery Algorithms in a Controlled Environment}
To establish a relation between the input quality and output quality, the in-vitro experiment is first prepared for the Inductive Miner.
As the algorithm is designed on process trees as the class of true process models, a random process tree generator is used for step 1 in the experiment.

Two settings have been used for the in-vitro experiment.
In both settings, the event logs were 10 times sampled for twelve sampling ratios: $0.01$, $0.02$, $0.05$, and $0.1$ up to $0.9$.
The first setting consisted of 10 models with each 10 original event logs with each 10,000 traces. In the second setting, 10 models were generated each with a single event log of 5,000 traces.

The results of the experiment are shown in Tbl.~\ref{tbl:run1} and~\ref{tbl:run2}.
The first setting resulted in 1200 samples per model.
For the analysis, each original log is first analyzed in isolation.
The Spearman rank correlation is calculated for each of the sample quality measures with precision and recall.
As each model has 10 event logs, Table~\ref{tbl:run1} reports the median for each model.

The second run generated 120 samples per model.
As the number of traces per event log is smaller, the event logs are less faithful representations of the true process than in the first run.
However, as Table~\ref{tbl:run1} shows, there is no clear correlation between the representativeness of the original event log and the results on the samples.

\begin{table}[t!]
	\begin{minipage}{\textwidth}
		\centering
		\caption{Results of setting 1. For each model 10 logs have been generated. Presented are the medians of each value. The last 8 columns show the Spearman rank correlation between the error measures, and precision and recall. Values in bold are statistically relevant ($p < 0.001$).}\label{tbl:run2}
		{\scriptsize
		\begin{tabular}{r|rr|rrrr|rrrr}

			& \multicolumn{2}{c|}{\textbf{True Process}} & \multicolumn{4}{c|}{\textbf{Precision}} & \multicolumn{4}{c}{\textbf{Recall}} \\\hline
			\textbf{Model} & \textbf{prec.} & \textbf{recall}           & sMAPE & sRMSPE & NRMSE & NMAE           & sMAPE & sRMSPE & NRMSE & NMAE \\\hline
			1  &           &                           &       &        &       &                &       &        &       &      \\
			2  &           &                           &       &        &       &                &       &        &       &      \\
			3  &           &                           &       &        &       &                &       &        &       &      \\
			4  &           &                           &       &        &       &                &       &        &       &      \\
			5  &           &                           &       &        &       &                &       &        &       &      \\
			6  &           &                           &       &        &       &                &       &        &       &      \\
			7  &           &                           &       &        &       &                &       &        &       &      \\
			8  &           &                           &       &        &       &                &       &        &       &      \\
			9  &           &                           &       &        &       &                &       &        &       &      \\
			10 &           &                           &       &        &       &                &       &        &       &      \\
		\end{tabular}
	}
	\end{minipage}
	\begin{minipage}{\textwidth}
	\vspace{1em}
	\centering
	\caption{Results of setting 2. The last 8 columns show the Spearman rank correlation between the error measures, and precision and recall. Values in bold are statistically relevant ($p < 0.001$).}\label{tbl:run1}
	{\scriptsize
	\begin{tabular}{r|rr|rrrr|rrrr}
                   & \multicolumn{2}{c|}{\textbf{True Process}} & \multicolumn{4}{c|}{\textbf{Precision}} & \multicolumn{4}{c}{\textbf{Recall}} \\\hline
	\textbf{Model} & \textbf{prec.} & \textbf{recall}           & sMAPE & sRMSPE & NRMSE & NMAE           & sMAPE & sRMSPE & NRMSE & NMAE \\\hline
	            1  & 0.538          &                           &       &        &       &                &       &        &       &      \\
	            2  & 0.797          &                           &       &        &       &                &       &        &       &      \\
	            3  & 0.935          &                           &       &        &       &                &       &        &       &      \\
	            4  & 0.953          &                           &       &        &       &                &       &        &       &      \\
	            5  & 0.988          &                           &       &        &       &                &       &        &       &      \\
	            6  & 0.871          &                           &       &        &       &                &       &        &       &      \\
	            7  & 0.943          &                           &       &        &       &                &       &        &       &      \\
	            8  & 0.616          &                           &       &        &       &                &       &        &       &      \\
	            9  & 0.710          &                           &       &        &       &                &       &        &       &      \\
	           10  & 0.883          &                           &       &        &       &                &       &        &       &      \\
%	           11  & 1.000          &                           &       &        &       &                &       &        &       &      \\
%	           12  & 0.772          &                           &       &        &       &                &       &        &       &      \\
%	           13  & 0.664          &                           &       &        &       &                &       &        &       &      \\
	\end{tabular}
}
	\end{minipage}
\end{table}

\subsection{Discusion of the Results}
The in-vivo experiments on both event logs show mixed results.
For precision, the Sepsis Case Log confirms the hypothesis that a better sample yields better results, whereas no such relation was found for recall.
For the road event logs no correlation or even a positive correlation was found between the eror measures and the conformance measures, indicating that a worse sample yields better results.

WHAT CAN WE CONCLUDE BASED ON THE RESULTS?

THE INDUCTIVE MINER IS A GOOD EXAMPLE THAT HAS SET INITIAL STEPS TOWARDS GUARANTEES: IT PROVIDES A CLASS OF TRUE PROCESSES, AND A CRITERION ON EVENT LOGS FOR REDISCOVERABILITY.
HOWEVER, NO MEASURES ARE GIVEN TO VALIDATE WHETHER AN EVENT LOG INDEED SATISFIES THE SET CRITERIA.
HOW DO YOU KNOW IF THE UNKNOWN TRUE PROCESS IS INDEED A PROCESS TREE, AND WHETHER THE EVENT LOG IS ACTIVITY COMPLETE? FOR THIS, A SET OF SUFFICIENT CRITERIA COULD BE STUDIED.
THIS LAST STEP WOULD THEN PROVIDE A SET OF GUARANTEES TO APPLY THE DISCOVERY ALGORITHM WITH MORE CERTAINTY.



==> section/designingOld.tex <==

RECIPE FOR ALGORITHM DESIGNERS, WHAT STEPS SHOULD THEY TAKE TO DESIGN AND PRESENT AN ALGORITHM

\subsection{Stage 0: Working Algorithm}

THERE IS SOME WORKING ALGORITHM

\subsection{Stage 1: Shown To Be Correct}

A. DESCRIBE THE CLASS OF TRUE PROCESS MODELS THAT GENERATES EVENT LOGS THE ALGORITHM WANTS AS INPUT

B. DEFINE THE CORRECTNESS GOAL OF THE ALGORITHM

C. SHOW THAT THE ALGORITHM SATISFIES THE GOAL, preferably with a formal proof.
(More difficult for an evolutionary algorithm)

\subsection{Stage 2: Algorithm is Validated}
IT SHOULD WORK ON SOME REAL EXAMPLES

\subsection{Stage 3: Established Relation Between Log Quality and Model Quality}
Upon introducing a new process discovery algorithm, authors now validate their algorithm on several real-life event logs, showing the possibilities of the algorithm.
However, these validations do not provide any guarantees on the qualities of the output of the algorithm.
In this paper, we propose a controlled experiment to systematically study the relationship between the quality of the inputs and outputs of a process discovery technique.
This \emph{in vitro} analysis allows algorithm designers to formulate guarantees of current and new discovery algorithms.


To study the guarantees a process discovery algorithm provides on the qualities of the output of the algorithm, we propose to perform an \emph{in vitro} analysis of the algorithm.
This in vitro analysis takes the form of a controlled experiment.
For the analysis, algorithm designers should first decide the class of process models for which they want to give guarantees.
For example, in~\cite{LeemansFA13}, the authors specifically design an algorithm for process trees.
The controlled experiment is outlined in Algorithm~\ref{algo:invitro}.
This class of process models are input of the controlled experiment, together with a set of sampling ratios, and the number of samples to assess per sampling ratio.
For each generated true process and corresponding event log, the precision and recall are used to quantify to what extent the event log is a faithful representation of the true process.
Then, similar to the \emph{in vivo} analysis, the quality of each sample is compared to the quality of the resulting process model.
Again, the Spearman rank correlation can be used for this.
In addition, the precision and recall of the original log can be used to study the relation between the representativeness of the original event log and the obtained sample qualities.


\begin{minipage}[t]{.48\textwidth}
\null 
\begin{algorithm}[H]
{\scriptsize
	\caption{InVitro}\label{algo:invitro}
\While{True}{
			$\mathit{TP} \gets$ GenerateModel($\mathcal{M}$, $A$)\;
			\ForEach{$i \in [1..N]$}{
				$L \gets$ GenerateLog($\mathit{TP}$, $T$)\;
				setModelQuality($L$, $\mathit{TP}$)\;
				\ForEach{$r \in \mathit{ratios}$}{
					\ForEach{$j \in [1..K]$}{
						$S \gets$ DrawSample($L$, $r$)\;
						setSampleQuality($L$, $S$)\;
						\BlankLine
						$M \gets$ DiscoverModel($S$)\;
						setModelQuality($S$, $M$)\;
					}
				}
			}
		}
	}
\end{algorithm}
\end{minipage}%
\begin{minipage}[t]{.48\textwidth}
\null
\begin{algorithm}[H]
	{\scriptsize
	\caption{InVivo}\label{algo:invivo}
	\ForEach{$r \in \mathit{ratios}$}{
		\ForEach{$j \in [1..K]$}{
			$S \gets$ DrawSample($L$, $r$)\;
			calculateSampleQuality($L$, $S$)\;
			\BlankLine
			$M \gets$ DiscoverModel($S$)\;
			calculatePrecisionAndRecall($S$, $M$)\;
		}
	}
}
\end{algorithm}
\end{minipage}

%
%\begin{minipage}{.49\textwidth}
%	\begin{algorithm}
%	\SetAlgoLined
%	\While{True}{
%		$\mathit{TP} \gets$ GenerateModel($\mathcal{M}$, $A$)\;
%		\ForEach{$i \in [1..N]$}{
%			$L \gets$ GenerateLog($\mathit{TP}$, $T$)\;
%			calculatePrecisionAndRecall($L$, $\mathit{TP}$)\;
%			%\For{$r \in \{0.01, 0.02, 0.05, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9 \}$}{
%			\ForEach{$r \in \mathit{ratios}$}{
%				\ForEach{$j \in [1..K]$}{
%					$S \gets$ DrawSample($L$, $r$)\;
%					calculateSampleQuality($L$, $S$)\;
%					\BlankLine
%					$M \gets$ DiscoverModel($S$)\;
%					calculatePrecisionAndRecall($S$, $M$)\;
%				}
%			}
%		}
%	}
%	\caption{InVitro Experiment}\label{algo:invitro}
%	\end{algorithm}
%\end{minipage}
%


\subsection{Stage 4: Algorithm is Effective}

In real-life situations, the true process that generated the event log is unknown.
In most process mining methods (cf.,~\cite{BozkayaGW09,EckLLA2015}) the event log is prepared, and then process discovery techniques are applied to unravel a process model.
An important question that these methods do not address is test-retest reliability: if the process is repeated on a new observation, i.e., a new event log, to what degree do the results agree between the analyses?
Now, the guarantees of a process discovery algorithm come into play.
If the different samples are of similar quality, then the constructed models should be of similar quality as well.
This requires an \emph{in vivo} approach to systematically validate the output of process discovery algorithms.


We propose a novel approach to assess process discovery results \emph{in vivo}.
The approach is outlined in Algorithm~\ref{algo:sampleLog}.
Given an event log $L$ and sampling ratio $r$, we draw a sample $S$, and calculate its error with respect to $L$.
As an example, the Inductive Miner~\cite{LeemansFA14} is used as discovery algorithm.
Last, Entropia~\cite{PolyvyanyyACGKL20} is used to calculate precision and recall of the sample and the discovered model.
The ranking of the samples based on the error measure is compared with the ranking of the samples based on each of the conformance measures.
If a process discovery algorithm treats correctness as a guarantee, than these ranks should be negatively correlated: a smaller error should result in a higher quality.
Hence, calculating Spearman's rank correlation on the error measures and the precision should result in a negative correlation.
The whole approach is implemented in ProM~\footnote{Source code available on: \url{https://github.com/ArchitectureMining/SamplingFramework}}.

%\begin{algorithm}[t]
%	\SetAlgoLined
%	\KwIn{Event Log $L$, set of ratios $\mathit{ratios}$, number of samples per ratio $K$}
%	\ForEach{$r \in \mathit{ratios}$}{
%		\ForEach{$j \in [1..K]$}{
%			$S \gets$ DrawSample($L$, $r$)\;
%			calculateSampleQuality($L$, $S$)\;
%			\BlankLine
%			$M \gets$ DiscoverModel($S$)\;
%			calculatePrecisionAndRecall($S$, $M$)\;
%		}
%	}
%	\caption{}\label{algo:sampleLog}
%\end{algorithm}



TWO LAYERS OF PROPERTIES AN ALGORITHM DESIGNER SHOULD TAKE INTO ACCOUNT:

1) IN VITRO

2) THE RESULTS SHOULD GENERALIZE TO IN VIVO, I.E., IF THE RESULTS HOLD IN VITRO, THEY SHOULD ALSO HOLD IN VIVO


Weak property:

For a specified class of true processes, there should be a negative Spearman rank correlation between error and the quality of the discovered model

Strong property:

For any two samples $S_1$ and $S_2$ of $L$, if $e(S_1) < e(S_2)$, then $\mathcal{P}^{S_1} > \mathcal{P}^{S_2}$.

Similar sample leads to similar model?



==> section/discussion.tex <==
this is a next step in data quality for process mining. previous studies only looked at things like missing or incomplete data.
We now lift the notion of log data quality to behavior.

The effect such methods and techniques have on process mining has never been studied. 
This results in the problem that it is impossible to generalize process mining results from samples. this framework sets a step in this direction. A Stage 4 algorithhm can generalize results from samples!
This is paper makes a step into this direction.

Why is it good to have such guarantees on conformance measures?

What is the difference with genetic / evolutionary algorithms?

we now enforce the last stage to the algorithm designers. 
another option is to extend process mining methods, to perform sampling on their event log, and use the experiment described in algo~\ref{algo:invivo} to establish and report confidence in the results they obtained.

ESTABLISH TRUST.
